Polyhedral Friction Cone Estimator for Object Manipulation

A polyhedral friction cone is a set of reaction wrenches that an object can experience whilst in contact with its environment. This polyhedron is a powerful tool to control an object's motion and interaction with the environment. It can be derived analytically, upon knowledge of object and environment geometries, contact point locations and friction coefficients. We propose to estimate the polyhedral friction cone so that a priori knowledge of these quantities is no longer required. Additionally, we introduce a solution to transform the estimated friction cone to avoid re-estimation while the object moves. We present an analysis of the estimated polyhedral friction cone and demonstrate its application for manipulating an object in simulation and with a real robot.

==> theory.tex <==
% ------------------------------------------------------------------------------------------
%                                   THEORY
%  
%   This section should make the following points clear to the reader.
%   * What is the polyhedron, what are its parameters, how does its parameters effect its shape.
%   * What happens at the edges of the polyhedron.
%   * What happens to the polyhedron as the block starts rotating.
%   * How could one achieve control knowing this polyhedron.
% ------------------------------------------------------------------------------------------

\subsection{Notation}
\label{subsec:notations}

In this paper we use both 2D and 3D vectors. To distinguish between the two, we use the notation $\vectwo{v}$ for vectors in $\R^2$ and $\vecthree{v}$ for vectors in $\R^3$.
We denote a normalised vector as $\hat{\vectwo{v}}$. We use $\rot{\phi}$ to denote the $2\! \times\! 2$ rotation matrix of angle $\phi$. We use $\vecthree{u}\times\vecthree{v}$ to denote the cross product between two 3D vectors; moreover, with the notation $\vectwo{u}\times\vectwo{v}$ we indicate the 3\textsuperscript{rd} component of the vector resulting from the cross product $(\vectwo{u}, 0)\times (\vectwo{v}, 0)$. Unless specified, all vectors are expressed in the wrench frame $\W$. We use $\vecbase{v}$ to denote a 2D vector in the base frame $\B$.


\subsection{Assumptions}
\label{subsec:assumptions}

We focus on a planar problem: in our system, objects are approximated with 2D shapes. Moreover, we consider polygonal objects, so that when moving in contact with the environment, a single contact point does not slide on the object's surface. 
We assume that the object's motion is sufficiently slow to consider the system quasi-static. The friction is modelled as Coulomb friction, and both object and environment are rigid. We approximate a line contact with two point contacts at its extremities.

We assume that the system begins operating with object and environment already in contact, but the object's geometry (in particular, the location of contact points) and the environment (in particular, the normals to its surfaces) are not known.

\subsection{Polyhedral friction cone}

\subsection{Reaction wrench space}
\label{subsec:reaction_wrench_space}

Consider an object and a frame of reference attached to it. If we apply a force to this object, it will produce a moment about the reference frame of the object. So, by combining both force and moment in a wrench vector, we can express the external force applied anywhere on the object as a wrench vector in the chosen frame of reference of the object. This can be regarded as a projection of a force vector in the 3D space to a wrench vector in a 6D space. Now, if the object makes contact with the environment at a single point, the object will experience a reaction force from the environment at the point of contact. As explained above, this reaction force can be expressed as a wrench vector in the chosen frame of reference of the object. We call this wrench a reaction wrench vector which lives in the 6D reaction wrench space. Note that, if the movements of the object and therefore the reaction forces are limited in a plane, the reaction wrench space will become three dimensional.


\subsection{Friction cone in reaction wrench space}
\label{subsec:friction_cone}

Assuming Coulomb friction between an object and the environment, the reaction force at each contact point is limited to the surface of the friction cone at that point. One can project this cone from the 3D space to the reaction wrench space in order to find the limits of the reaction wrench vector.

In the case of a planar motion, the friction cone at a contact point becomes a triangle which lies in the plane of motion. This friction triangle defines the limits of the reaction force at the point of contact. As an example, Figure~\ref{fig:block_point_contact}(a) shows a rectangular block which has a one-point contact at $A$ with the horizontal surface. Right and left sides of the friction triangle at this point is shown by $\vecbase{f}_r$ and $\vecbase{f}_l$, respectively. Projections of these two vectors from the motion plane to the 3D reaction wrench space are the limits of the wrench vector in that space. Let $\vectwo{p}_A$ denote the position of the contact point $A$ in frame $\W$ which is our chosen reference frame. This frame which is shown in Fig.~\ref{fig:block_point_contact}(a) is aligned with the principal axes of the block and attached to its centre. 
%
\begin{figure}
  \centering
  \begin{tabular}{cc}
    \includegraphics[trim={0.5cm 0cm 2cm 0cm},clip, scale=0.48]{figures/block_one_contact.png} &
    \includegraphics[trim={16cm 0.5cm 14cm 8.5cm},clip, scale=0.25]{figures/friction_cone_wrench.png}\\
    (a) & (b)
  \end{tabular}
  \caption{(a) A rectangular block in contact with the horizontal surface at point $A$. (b) projection of the friction cone at $A$ in the reaction wrench space.}
  \label{fig:block_point_contact}
\end{figure}
%
The wrench vectors corresponding to $\vecbase{f}_r$ and $\vecbase{f}_l$ in the wrench space of frame $\W$ are
%
\begin{equation}
    \label{eq:wrench_fr_fl}
    \begin{split}
        \vecthree{w}_r & = (\vectwo{f}_r, \, \vectwo{p}_A \times \vectwo{f}_r) \\
        \vecthree{w}_l & = (\vectwo{f}_l, \, \vectwo{p}_A \times \vectwo{f}_l) \, ,
    \end{split}
\end{equation}
%
where
%
\begin{equation}
    \vectwo{f} = \mathbf{R}^T(\phi) \, \vecbase{f}
\end{equation}
%
and $\phi$ is the angle of rotation of frame $\W$ with respect to the base frame.

Figure~\ref{fig:block_point_contact}(b) shows $\vecthree{w}_r$ and $\vecthree{w}_l$ in the reaction wrench space of frame $\W$. These two vectors construct a plane in this space. Note that, any possible reaction wrench at point $A$ always lies in this plane and in the surface between $\vecthree{w}_r$ and $\vecthree{w}_l$. It can be proved that (depends on where we put the proof) the direction of the normal to this plane is a function of $\vectwo{p}_A$ and independent of the rotation angle (i.e. $\phi$) of the block. It means that, if the block rotates about the contact point $A$, the surface that defines the limits of the reaction wrench always remains on the same plane. We call this plane the \textit{friction cone plane} of $A$ in the reaction wrench space. 


\subsection{Polyhedral friction cone}
\label{subsec:polyhedral}

If the block in Fig.~\ref{fig:block_point_contact}(a) makes a contact with the horizontal surface at point $B$, the friction cone at $B$ will have a corresponding triangular surface on the friction cone plane of $B$ in the reaction wrench space. Since $\vectwo{p}_B$ is different from $\vectwo{p}_A$, the friction cone planes of $A$ and $B$ will be different. Figure~\ref{fig:block_surface_contact} (a) shows the block which has contacts at both $A$ and $B$. The projected friction cones at these two points in the reaction wrench space are shown in Fig.~\ref{fig:block_surface_contact} (b).
%
\begin{figure}
  \centering
  \begin{tabular}{cc}
    \includegraphics[trim={1.2cm 0cm 0cm 0cm},clip, scale=0.7]{figures/block_surface_contact.png} &
    \includegraphics[trim={15cm 7cm 9cm 8.5cm},clip, scale=0.35] {figures/polyhedral.png}\\
    (a) & (b)
  \end{tabular}
  \caption{(a) The rectangular block in a surface contact with the horizontal plane, and (b) its corresponding polyhedral friction cone.}
  \label{fig:block_surface_contact}
\end{figure}
%
The vectors of the edges of the projected friction cones are represented by four vectors $\vecthree{w}_{r_A}$, $\vecthree{w}_{l_A}$, $\vecthree{w}_{r_B}$, $\vecthree{w}_{l_B}$. These vectors are computed using (\ref{eq:wrench_fr_fl}) for both $A$ and $B$. These four vectors construct a polyhedral convex shape in the reaction wrench space. It is known that, as long as the contacts at $A$ and $B$ are maintained, any reaction wrench will be limited to this polyhedral. This convex shape is called \textit{polyhedral friction cone} in this paper.


\subsection{Relation to the modes of motion}
\label{subsec:motion_modes}

Consider the block in Fig.~\ref{fig:block_surface_contact} (a) which is in a surface contact with the environment at $AB$. Let $\vecthree{w}_r$ denote the reaction wrench that is applied to the block from the environment and $\vecthree{w}_a$ denote the \textit{action} wrench that is exerted on the block by other means including control input and the gravity. When the block is in static equilibrium, $\vecthree{w}_a + \vecthree{w}_r = 0$, which means that $\vecthree{w}_r$ is equal and in the opposite direction of $\vecthree{w}_a$. However, if $\vecthree{w}_a + \vecthree{w}_r \neq 0$, the difference between $\vecthree{w}_r$ and $-\vecthree{w}_a$ will create an acceleration on the block and breaks its static equilibrium. 

During the movement of the block the reaction wrench always stays on the surface of the polyhedral friction cone. This is because $-\vecthree{w}_a$ is outside of the polyhedral and is pulling $\vecthree{w}_r$ to its limits. The type of movement of the block depends on where $\vecthree{w}_r$ meets the surface of the polyhedral friction cone. Since, in our example, the polyhedral consists of four lateral edges and four lateral surfaces, there will be eight possibilities in total for the movement of the block. Four of them, which are the main modes of motion and correspond to the four lateral surfaces, are sliding right, sliding left, pivoting counter-clockwise on $A$ and pivoting clockwise on $B$. The corresponding four surfaces of the polyhedral in Fig.~\ref{fig:block_surface_contact} (b) are labelled by \srSurface{}, \slSurface{}, \ccwSurface{}  and \cwSurface{}, respectively. The other four modes of motion are actually a set of combination of sliding and pivoting motions which happen when the reaction wrench is at the lateral edges of the polyhedral. These modes, which are called \textit{mixed modes} of motion in this paper, are pivoting counter-clockwise on $A$ and sliding right, pivoting counter-clockwise on $A$ and sliding left, pivoting clockwise on $B$ and sliding right and pivoting counter-clockwise on $B$ and sliding left. The corresponding edges in Fig.~\ref{fig:block_surface_contact} (b) are denoted by $\vecthree{w}_{r_A}$, $\vecthree{w}_{l_A}$, $\vecthree{w}_{r_B}$ and $\vecthree{w}_{l_B}$, respectively.

When the block starts to rotate, either counter-clockwise about $A$ or clockwise about $B$, it loses contact at the other point. Therefore, the polyhedral will lose the corresponding two lateral edges, due to the loss of contact, and becomes a triangle as mentioned in \ref{subsec:friction_cone}. In this case, there still exist the same eight possible modes of motion for the block. However, there are only three possibilities for the reaction wrench: it is either on the left or right side of the triangle or it lies in the area between the two. These three cases correspond to sliding left, sliding right and no sliding, respectively. Therefore, there is not any one-to-one mapping from the reaction wrench to the modes of motion when there is one point of contact. Although, in this case, we can relate the modes of motion to the location of $-\vecthree{w}_a$ with respect to the friction triangle in the reaction wrench space.

Figure~\ref{fig:action_wrench_labels} shows the friction triangle for the block when it is in a point contact at $A$. In this figure, similar to Fig.~\ref{fig:block_point_contact} (b), the friction triangle is represented by the area between $\vecthree{w}_r$ and $\vecthree{w}_l$ on the friction cone plane. If $-\vecthree{w}_a$ lies on this plane and outside of the friction triangle, no out-of-plane wrench will be exerted to the block and the block will slide to either left or right. The corresponding areas in the wrench space are shown by \srSurface{} and \slSurface{} in Fig.~\ref{fig:action_wrench_labels}. If $-\vecthree{w}_a$ is outside of the friction cone plane but inside the normal extension of the friction triangle, $\vecthree{w}_r$ will stay inside the friction triangle. Therefore, the block will experience a pure rotation either clockwise or counter-clockwise. The corresponding areas are labelled by \cwSurface{} and \ccwSurface{} in Fig.~\ref{fig:action_wrench_labels}.
Mixed modes of motion will be achieved if $-\vecthree{w}_a$ lies in the area connecting the main modes in the reaction wrench space. These areas are labelled by \cwsrEdge{}, \ccwsrEdge{}, \cwslEdge{} and \ccwslEdge{} in Fig.~\ref{fig:action_wrench_labels}.
%
\begin{figure}
  \centering
  \includegraphics[trim={1cm 1cm 4cm 6cm},clip, scale=0.25]{figures/action_wrench_label.png}
  \caption{Reaction wrench space divisions and corresponding labels based on the location of $-\vecthree{w}_a$ with respect to the projection of the friction cone at the contact point $A$.}
  \label{fig:action_wrench_labels}
\end{figure}
%
